PRNet: Self-Supervised Learning for Partial-to-Partial Registration

We present a simple, flexible, and general framework titled Partial Registration Network (PRNet), for partial-to-partial point cloud registration. Inspired by recently-proposed learning-based methods for registration, we use deep networks to tackle non-convexity of the alignment and partial correspondence problems. While previous learning-based methods assume the entire shape is visible, PRNet is suitable for partial-to-partial registration, outperforming PointNetLK, DCP, and non-learning methods on synthetic data. PRNet is self-supervised, jointly learning an appropriate geometric representation, a keypoint detector that finds points in common between partial views, and keypoint-to-keypoint correspondences. We show PRNet predicts keypoints and correspondences consistently across views and objects. Furthermore, the learned representation is transferable to classification.

==> section/ablation.tex <==
\section{Ablation Study}

\begin{table}
% \vskip -0.3in
\begin{minipage}[t]{0.5\textwidth}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Method & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$  & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
Random sampling & 1.689 & 0.927 & 0.011 & \textbf{0.997} \\
Closeness to other points  & 2.109 & 0.861 & 0.013 & 0.995 \\
$L^2$ Norm & \textbf{1.454} & \textbf{0.939} & \textbf{0.010} & \textbf{0.997} \\
\bottomrule
\end{tabular}
}
(\ca) Different keypoint detection methods.\label{keypoint:detection}
\end{center}
% \vskip -0.4in
\end{minipage}
%
\begin{minipage}[t]{0.5\textwidth}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Different $k$ & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$  & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
16 & 27.843 & -14.176 & 0.136 & 0.326\\
32 & 8.293 & -1.848 & 0.048 & 0.892\\
64 & 3.129 & 0.563 & 0.024 & 0.979 \\
128 & 2.007 & 0.879 & 0.016 & 0.991\\
256 & 1.601 & 0.932 & 0.012 & 0.996\\
384 & 1.508 & 0.934 & 0.011 & \textbf{0.997}\\
512  & \textbf{1.454} & \textbf{0.939} & \textbf{0.010} & \textbf{0.997} \\
\bottomrule
\end{tabular}
}
(\cd) Different number of keypoints ($k$).\label{keypoint:differentk}
\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.5\textwidth}
% \vskip -0.66in
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Model & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$  & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
ICP & 25.165 & -5.860 & 0.250 & -0.045 \\
Go-ICP & 2.336 & 0.308 & 0.007 & 0.994\\
FGR  & 2.088 & 0.393  & \textbf{0.003} & 0.999\\
PointNetLK  & 3.478 & 0.051 & 0.005 & 0.994\\
DCP &  2.777 & 0.887 & 0.009 & 0.998 \\
\midrule
PRNet (Ours) &  \textbf{0.960} & \textbf{0.979} & 0.006 & \textbf{1.000} \\
\bottomrule
\end{tabular}
}
(\cb) Experiments on full point clouds. \label{fullscan} 
\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.5\textwidth}
% \vskip -1.0in
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Data Missing Ratio & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$ & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
75\% & 6.447 & 0.028 & 0.042 & 0.921 \\
50\% & 3.939 & 0.623 & 0.0288 & 0.969 \\
25\% & \textbf{1.454} & \textbf{0.939} & \textbf{0.010} & \textbf{0.997} \\
\bottomrule
\end{tabular}
}
(\ce) Data missing ratio. \label{datamissing:ratio}
% \vskip -2.0in
\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.5\textwidth}
% \vskip -0.1in
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Discount Factor $\lambda$ & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$ & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
0.5 & 1.921 & 0.917 & 0.014 & 0.995\\
0.7 & 1.998 & 0.884 & 0.014 & 0.995\\
0.9 & \textbf{1.454} & \textbf{0.939} &  \textbf{0.010} & \textbf{0.997} \\
0.99 & 1.732 & 0.915  & 0.012 & 0.996\\
\bottomrule
\end{tabular}
}
(\cc) Different discount factors ($\lambda$). \label{discountfactor} 
\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.5\textwidth}
% \vskip -0.55in
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Data Noise & MAE($\bR$) $\downarrow$ & R$^2$($\bR$) $\uparrow$ & MAE($\bt$) $\downarrow$ & R$^2$($\bt$) $\uparrow$\\ 
\midrule
$\N(0, 0.01^2)$  & \textbf{2.051} & \textbf{0.889} & \textbf{0.012} & \textbf{0.995} \\
$\N(0, 0.1^2)$  & 5.013 & 0.617 & 0.020 & 0.991 \\
$\N(0, 0.5^2)$  & 21.129 & -2.830 & 0.064 & 0.917 \\
\bottomrule
\end{tabular}
}
(\cf) Data noise. \label{datanoise}
\end{center}
\end{minipage}
\caption{Ablation studies.\label{ablation}}
% \vskip -0.4in
\end{table}
\textbf{Keypoint detection alternatives, experiments on full point clouds, effects of discount factor, choice of $k$, robustness to data missing ratio, robustness to data noise.} To understand the effectiveness of each part, we conduct additional experiments in Table~\ref{ablation}; to save space, we only show MAE and R$^2$. (\ca) First, we consider alternatives to keypoint selection: in the first alternative, the two sets of keypoints are chosen independently and randomly on the two surfaces ($\X$ and $\Y$); 
in the second alternative, we use \emph{centrality} to choose keypoints, keeping the $k$ points whose average distance (in feature space) to the rest in the point cloud is minimal. Empirically, the $L^2$ norm used in our pipeline to select keypoints outperforms others. 
(\cb) Second, we compare our method to others on full point clouds. In this experiment, 768 points are sampled from each point cloud to cover the full shape using farthest-point sampling. In the full point cloud setting, PRNet still outperforms others.
(\cc) Third, we verify our choice of discount factor $\lambda$; small large discount factors encourage alignment within the first few passes through PRNet while large discount factors promote longer-term return. 
(\cd) Fourth, we test the choice of number of keypoints: the model achieves surprisingly good performance even with 64 keypoints, but performance drops significantly when $k<32$. 
(\ce) Fifth, we test its robustness to missing data. The missing data ratio in original partial-to-partial experiment is 25\%; we further test with 50\% and 75\%. This test shows that with 75\% points missing, the method still achieves reasonable performance, even compared to other methods tested with only 25\% points missing.
(\cf) Finally, we test the model robustness to noise level. Noise is sampled from $\N(0, \sigma^2)$. The model is trained with $\sigma=0.01$ and tested with $\sigma \in [0.01, 0.1, 0.5]$. Even with $\sigma=0.1$, the model still performs reasonably well. 
\begin{wraptable}[11]{l}{0.45\linewidth}
\begin{center}
\vskip -0.2in
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccr}
\toprule
\# points & ICP & Go-ICP & FGR  & PointNetLK & DCP & PRNet\\ 
\midrule
512 & 0.134 & 14.763 & 0.230 & 0.049 & 0.014 & 0.042 \\
1024 & 0.170  & 14.853 & 0.250 & 0.061  & 0.024 & 0.073\\
2048 & 0.242 & 14.929 & 0.248 & 0.069  & 0.058 & 0.152\\
\bottomrule
\end{tabular}
}
\end{center}
% \vskip -0.15in
% \caption{Inference time (in seconds). \label{efficiency}}
\vskip -0.3in
\end{wraptable}

\textbf{Alternatives to Gumbel-Softmax.} Methods to tackle non-differentiability usually fall into two categories: REINFORCE and Gumbel-Softmax. REINFORCE produces unbiased high-variance gradient estimation while Gumbel-Softmax produces biased gradients with low variance. Empirically, we tried vanilla REINFORCE to estimate the gradients of the matching function; due to its instability, the training did not converge. Studying unbiased low-variance gradient estimation is extremely valuable to reinforcement learning and/or discrete optimization, but introducing complicated gradient estimator is beyond the scope of this paper. \\
\textbf{Efficiency.} We benchmark the inference time of different methods on a desktop computer with an Intel 16-core CPU, an Nvidia GTX 1080 Ti GPU, and 128G memory. Table~\ref{efficiency} shows learning based methods (on GPUs) are faster than non-learning based counterparts (on CPUs). PRNet is on a par with PointNetLK while being slower than DCP. 

